Robust PDF Files Forensics Using Coding Style

Identifying how a file has been created is often interesting in security. It can be used by both attackers and defenders. Attackers can exploit this information to tune their attacks and defenders can understand how a malicious file has been created after an incident. In this work, we want to identify how a PDF file has been created. This problem is important because PDF files are extremely popular: many organizations publish PDF files online and malicious PDF files are commonly used by attackers. Our approach to detect which software has been used to produce a PDF file is based on coding style: given patterns that are only created by certain PDF producers. We have analyzed the coding style of 900 PDF files produced using 11 PDF producers on 3 different Operating Systems. We have obtained a set of 192 rules which can be used to identify 11 PDF producers. We have tested our detection tool on 508836 PDF files published on scientific preprints servers. Our tool is able to detect certain producers with an accuracy of 100%. Its overall detection is still high (74%). We were able to apply our tool to identify how online PDF services work and to spot inconsistency.

==> dataset.tex <==
\section{Dataset}\label{sec:meta}
To check the adoption of PDF sanitization, we have chosen to work on the PDF files published by different security agencies around the world and scientific community associated to research work. In this section, we describe our datasets and the level of sanitization followed by these two entities.

The National Security Agency (NSA) is one of the main actor in cyber security and it has provided many guidelines to sanitize PDF files before sharing them~\cite{NSA2005,NSA2008,NSA2015}.  This was one of the motivations in our work to check if security agencies around the world also sanitize their PDF files before publication or not. Research community regularly deals with PDF files to publish and share their work. Researchers are supposed to be well aware of the PDF metadata and the privacy issues associated to information leakage.  We wanted to check how important is sanitization for both security agencies and researchers.

% sanitize their PDF files before publication.

\subsection{Dataset}
We have downloaded PDF files from the websites of security agencies and preprints of scientific community.

\textbf{Security agencies}: We have crawled the websites of 75 security agencies mentioned by Wikipedia\footnote{\url{https://en.wikipedia.org/wiki/Security\_agency}} belonging to 47 countries. We downloaded 39664 PDF files in total. The distribution of PDF files over the agency is not even. We found between 5 to around 6000 PDF files for each agency. Figure~\ref{fig:dataset} in Appendix~\ref{sec:appendix} shows the discrepancy in the number of PDF files for each country in our dataset.

\textbf{preprints of scientific community}: Conference proceedings and preprint are clearly the best options to obtain PDF files on a large scale. Our second dataset was downloaded from the Cryptology ePrint Archive\footnote{\url{https://eprint.iacr.org/}}, it includes 11405 PDF documents from 2004 to 2018. Open archive HAL\footnote{\url{https://hal.archives-ouvertes.fr/}} administrators provided us with an access to a third set of dataset of PDF files. It consists of 544460 PDF files from 1996 to 2019. 

HAL provides options to either directly submit a PDF file or submit source files and create a PDF file using HAL's pdf producer tool \texttt{PdfLaTeX}. We observed that around 47\% of the PDF files in HAL dataset were compiled by HAL while the rest 53\% were originally compiled by the author(s) using a PDF producer tool of there choice.  All the PDF files submitted to HAL are concatenated with a cover page using Apache PDFBOX. Hence all the PDF files published are modified. \\

Our datasets are respectively called Security dataset, IACR dataset and HAL dataset throughout the paper for convenience. 


%We observed that all the PDF documents were originally compiled by the authors using a PDF producer tool of their choice. They are respectively called IACR dataset and HAL dataset throughout the paper for convenience. The IACR and HAL PDF files are not anonymous, \textit{i.e.} they include the name of the author(s). Also, it is possible to find a description (metadata) of author names, title, year of publication of each PDF file on there respective websites.

%We observed that the metadata of 53\% of the PDF files in HAL dataset are likely to be original values of authors PDF producer tools. For the rest of the HAL's PDF files, we have clues that metadata were altered by HAL. We have considered all these PDF files in HAL dataset for our experiments.

